Evaluate Summarization in Fine-Granularity: Auto Evaluation with LLM

Due to the exponential growth of information and the need for efficient information consumption the task of summarization has gained paramount importance. Evaluating summarization accurately and objectively presents significant challenges, particularly when dealing with long and unstructured texts rich in content. Existing methods, such as ROUGE (Lin, 2004) and embedding similarities, often yield scores that have low correlation with human judgements and are also not intuitively understandable, making it difficult to gauge the true quality of the summaries. LLMs can mimic human in giving subjective reviews but subjective scores are hard to interpret and justify. They can be easily manipulated by altering the models and the tones of the prompts. In this paper, we introduce a novel evaluation methodology and tooling designed to address these challenges, providing a more comprehensive, accurate and interpretable assessment of summarization outputs. Our method (SumAutoEval) proposes and evaluates metrics at varying granularity levels, giving objective scores on 4 key dimensions such as completeness, correctness, Alignment and readability. We empirically demonstrate, that SumAutoEval enhances the understanding of output quality with better human correlation.

==> section2.1-overview.tex <==
\section{Overview}
\textcolor{red}{Eti - is it still needed???}
To evaluate a long-text summary thoroughly in fine-granularity, we first need to extract entities from ground truth note and target note as described in Section~\ref{entity_extraction}.

{\bf Entity} is defined as a short phrase that contains one and only one key concept.

Based on the extracted entities, we designed methods to evaluate the metrics defined in Section \ref{metrics}.
With the summary and extracted entities, we do both entity and paragraph-level quality detection to measure summary's quality.
%1. Rubric Note/Target Note Entity Extraction

%Output: (entity, entity\_reference(optional), entity\_context)
To evaluate the completeness of the summary, we evaluate the missing entities ratio in ground truth note that are not in the target note, namely the missing count (Section \ref{method:missing}).

To evaluate the correctness of a note, we evaluate the ratio of entities in the target note that are wrong.

To evaluate...



Finally, we... Aggregation/Mapping to Final Metrics


